TensoRF: Tensorial Radiance Fields

We present TensoRF, a novel approach to model and reconstruct radiance fields. Unlike NeRF that purely uses MLPs, we model the radiance field of a scene as a 4D tensor, which represents a 3D voxel grid with per-voxel multi-channel features. Our central idea is to factorize the 4D scene tensor into multiple compact low-rank tensor components. We demonstrate that applying traditional CP decomposition -- that factorizes tensors into rank-one components with compact vectors -- in our framework leads to improvements over vanilla NeRF. To further boost performance, we introduce a novel vector-matrix (VM) decomposition that relaxes the low-rank constraints for two modes of a tensor and factorizes tensors into compact vector and matrix factors. Beyond superior rendering quality, our models with CP and VM decompositions lead to a significantly lower memory footprint in comparison to previous and concurrent works that directly optimize per-voxel features. Experimentally, we demonstrate that TensoRF with CP decomposition achieves fast reconstruction (<30 min) with better rendering quality and even a smaller model size (<4 MB) compared to NeRF. Moreover, TensoRF with VM decomposition further boosts rendering quality and outperforms previous state-of-the-art methods, while reducing the reconstruction time (<10 min) and retaining a compact model size (<75 MB).

==> tex/method-bk.tex <==
\newcommand{\Tensor}{\mathcal{T}}
\newcommand{\Vector}{\mathbf{v}}
\newcommand{\Matrix}{\mathbf{M}}
\newcommand{\AppVec}{\mathbf{b}}
\newcommand{\AppMat}{\mathbf{B}}
\newcommand{\VectorPack}{\mathbf{V}}
\newcommand{\RRR}{\mathbb{R}}
\newcommand{\DimIJK}{I\times J\times K}
\newcommand{\DimCh}{P}


\newcommand{\OuterP}{\circ}
\newcommand{\ScalarP}{\ast}
\newcommand{\Pos}{\mathbf{x}}
\newcommand{\Dens}{\sigma}
\newcommand{\Rad}{c}
\newcommand{\Comp}{\mathcal{A}}
\newcommand{\Dir}{d}
\newcommand{\Grid}{\mathcal{G}}
\newcommand{\ShadFunc}{S}



\section{Vector-Matrix Factorization.}
\label{sec:vm-factor}
Our approach factorizes a feature grid-based radiance field into compact components.
While standard tensor decompositions can be applied, we introduce a new vector-matrix decomposition, facilitating the radian field reconstruction and rendering.
We now review the classical CP decomposition and present our decomposition for the case of a 3D (3rd-order) tensor. We will introduce how to apply the decomposition in radiance field modeling in Sec.~\ref{sec:tensorf}.

\paragraph{CP decomposition.} Given a 3D tensor $\Tensor \in \RRR^{I\times J\times K}$, CP decomposition factorizes it into a sum of outer products of vectors:
\begin{equation}
    \Tensor = \sum_{r=1}^R \Vector_r^{1} \OuterP \Vector_r^{2} \OuterP \Vector_r^{3},
    \label{eqn:cpvector}
\end{equation}
where $\Vector_r^{1} \OuterP \Vector_r^{2} \OuterP \Vector_r^{3}$ corresponds to a rank-one tensor component, and $\Vector_r^{1} \in \RRR^{I}$, $\Vector_r^{2} \in \RRR^{J}$, and $\Vector_r^{3} \in \RRR^{K}$ are factorized vectors of the three modes for the $r$th component. Superscripts denote the modes of each factor in this paper. $OuterP$ denotes the outer product. This leads to each tensor element $\Tensor_{ijk}$ computed by
\begin{equation}
    \Tensor_{ijk} = \sum_{r=1}^R \Vector_{r,i}^{1} \ScalarP \Vector_{r,j}^{2} \ScalarP \Vector_{r,k}^{3},
    \label{eqn:cpelement}
\end{equation}
where $i$, $j$, $k$ denote the indices of the three modes respectively, and $\ScalarP$ represents scalar multiplication.

Essentially, CP decomposition factorizes a tensor to multiple vectors, expressing multiple compact rank-one components. 
We show that CP can be also applied in our tensorial radiance field modeling and generate reasonable rendering results. However, while leading to very high compactness, CP decomposition can require many components to reach high accuracy, burdening the extensive computation in radiance field reconstruction.
Inspired by CP and block term decomposition (BTD), we present a new decomposition that leads to efficient radiance field reconstruction.

\paragraph{Vector-Matrix decomposition.} Unlike CP decomposition that leads to pure vector factors, our decomposition factorizes a tensor into multiple vectors and matrices. This is expressed by
\begin{equation}
    \Tensor = \sum_{r=1}^{R_1} \Vector_r^{1} \OuterP \Matrix_r^{2,3} + \sum_{r=1}^{R_2}\Vector_r^{2} \OuterP \Matrix_r^{1,3} + \sum_{r=1}^{R_3}\Vector_r^{3} \OuterP \Matrix_r^{1,2} 
    \label{eqn:vmrrr}
\end{equation}
where $\Matrix_r^{2,3} \in \RRR^{J\times K}$, $\Matrix_r^{1,3} \in \RRR^{I\times K}$, $\Matrix_r^{1,2} \in \RRR^{I\times J}$ are matrix factors for two (denoted by its superscripts) of the three modes.
Basically, for each component tensor, we relax its two mode ranks to be arbitrarily large, while fixing the third mode rank to be one; e.g., for component tensor $\Vector_r^{1} \OuterP \Matrix_r^{2,3}$, its mode-1 rank is 1, while its mode-2 and mode-3 ranks can be arbitrary,depending on the rank of the matrix $\Matrix_r^{2,3}$.
Essentially, each of our component tenor has many more parameters than a component in CP decomposition. 
While this leads to lower compactness, our decomposition requires significantly fewer number of components in radiance field modeling, leading to highly efficient scene reconstruction.

We alternate the two modes for the matrix factor to allow each mode to be adequately parametrized. In most cases, we also set $R_1=R_2=R_3=R$; in the context of 3D scene representation, this reflects the fact that a scene can distribute and appear equally complex along its three axes. This leads to a reduced version of Eqn.~\ref{eqn:vmrrr}
\begin{equation}
    \Tensor = \sum_{r=1}^{R} \Vector_r^{1} \OuterP \Matrix_r^{2,3} + \Vector_r^{2} \OuterP \Matrix_r^{1,3} + \Vector_r^{3} \OuterP \Matrix_r^{1,2}, 
    \label{eqn:vmr}
\end{equation}
and its element-wise format is expressed by
\begin{equation}
    \Tensor_{ijk} = \sum_{r=1}^{R} \Vector_{r,i}^{1} \ScalarP \Matrix_{r,jk}^{2,3} + \Vector_{r,j}^{2} \ScalarP \Matrix_{r,ik}^{1,3} + \Vector_{r,k}^{3} \ScalarP \Matrix_{r,ij}^{1,2}, 
    \label{eqn:vmrelement}
\end{equation}

Our vector-matrix decomposition can be seen as a special case of BTD and is also similar to a rank-(L,L,1) BTD. Unlike rank-(L,L,1) BTD, we do not constrain the rank of a matrix factor and we alternate the tensor modes for the matrix in different components, facilitating the task of radiance field reconstruction. 

\section{TensoRF Representation}
\label{sec:tensorf}
We present our tensorial radiance field representation.

\subsection{Feature grids and radiance fields.}
\label{sec:grids}
Our goal is to model a radiance field, which is essentially a function that maps any 3D location $\Pos$ and viewing direction $\Dir$ to its volume density $\Dens$ and view-dependent color $\Rad$, supporting differentiable ray marching for volume rendering.
We leverage a regular 3D grid $\Grid$ with per-voxel multi-channel features to model such a function.
We split it (by feature channels) to a geometry grid $\Grid_\Dens$ and an appearance grid $\Grid_\Rad$, which separately model the volume density and view-dependent color.

Our approach supports general types of appearance features in $\Grid_\Rad$, depending on a pre-selected shading function $\ShadFunc$ that coverts an appearance feature vector and a viewing direction $\Dir$ to color $\Rad$. We show that $\ShadFunc$ can be a small MLP or spherical harmonics (SH) functions, where $\Grid_\Rad$ contains neural features and SH coefficients respectively. 
On the other hand, we consider a single-channel grid $\Grid_\Dens$, whose values represent volume density directly, without requiring an extra converting function. In general, a continuous grid-based radiance field can be written as
\begin{equation}
    \Dens, \Rad = \Grid_\Dens(\Pos), \ShadFunc(\Grid_\Rad(\Pos),\Dir),
    \label{eqn:rf}
\end{equation}
where $\Grid_\Dens(\Pos)$, $\Grid_\Rad(\Pos)$ represent the trilinearly interpolated features from the two grids at location $\Pos$. 
We consider $\Grid_\Dens$ and $\Grid_\Rad$ as tensors, and factorize them for modeling.

\subsection{Factorizing radiance fields}
In essence, $\Grid_\Dens \in \RRR^{\DimIJK}$ is a 3D tensor and $\Grid_\Rad \in \RRR^{\DimIJK\times \DimCh}$ is a 4D tensor; here $I$, $J$, $K$ corresponds to the resolutions of the feature grid along the X, Y, Z axes, and $\DimCh$ is the number of appearance feature channels. 

We propose to factorize these radiance field tensors to vectors and matrices using the techniques described in Sec.~\ref{sec:vm-factor}
In particular, the geometry tensor $\Grid_\Dens$ is factorized into by vectors $\Vector_{\Dens, r}^{X}$, $\Vector_{\Dens, r}^{Y}$, $\Vector_{\Dens, r}^{Z}$, and matrices $\Matrix_{\Dens,r}^{YZ}$, $\Matrix_{\Dens,r}^{XZ}$, $\Matrix_{\Dens,r}^{XY}$, for $r=1,..,R_\Dens$. Here, since the modes of our tensors correspond to the coordinate frame, we directly use $X$, $Y$, $Z$ to denote the three modes. These vector and matrix factors essentially describe the spatial variations of the scene geometry (volume density) along their corresponding axes. 
% Similar to Eqn.~\ref{eqn:vmrelement}, each grid element is computed by
% \begin{equation}
%     \Grid_{\Dens,ijk} = \sum_{r=1}^{R} \Vector_{\Dens r,i}^{X} \Matrix_{\Dens r,jk}^{Y,Z} + \Vector_{\Dens r,j}^{Y} \Matrix_{\Dens r,ik}^{X,Z} + \Vector_{\Dens r,k}^{Z} \Matrix_{\Dens r,ij}^{X,Y}. 
%     \label{eqn:dense-vmr}
% \end{equation}
The factorization is expressed as
\begin{equation}
    \Grid_{\Dens} = \sum_{r=1}^{R_\Dens} \Vector_{\Dens, r}^{X} \OuterP \Matrix_{\Dens,r}^{YZ} + \Vector_{\Dens,r}^{Y} \OuterP \Matrix_{\Dens,r}^{XZ} + \Vector_{\Dens,r}^{Z} \OuterP \Matrix_{\Dens,r}^{XY}. 
    \label{eqn:dense-vmr}
\end{equation}

% We also denote tensor components $\Comp_{\Dens,r}^X=\Vector_{\Dens, r}^{X} \OuterP \Matrix_{\Dens,r}^{YZ}$, $\Comp_{\Dens,r}^Y=\Vector_{\Dens, r}^{Y} \OuterP \Matrix_{\Dens,r}^{XZ}$, $\Comp_{\Dens,r}^Z=\Vector_{\Dens, r}^{Z} \OuterP \Matrix_{\Dens,r}^{XY}$.

The appearance tensor $\Grid_\Rad$ has an additional mode corresponding to the feature channel dimension. Note that, compared to XYZ modes, this mode is often of a lower rank, since its dimension is generally lower. Therefore, we do not combine this mode with other modes in matrix factors and instead only use vectors, denoted by $\AppVec_r$, for this mode in the factorization. 
Specifically, $\Grid_\Rad$ is factorized into $\Vector_{\Rad, r}^{X}$, $\Vector_{\Rad, r}^{Y}$, $\Vector_{\Rad, r}^{Z}$, $\Matrix_{\Rad,r}^{YZ}$, $\Matrix_{\Rad,r}^{XZ}$, $\Matrix_{\Rad,r}^{XY}$, for $r=1,..,R_\Rad$, and $\AppVec_r$, for $r=1,..,3R_\Rad$. Note that, we need to have $3R_\Rad$ vectors $\AppVec_r$ to match the total number of components. In particular, $\Grid_\Rad$ is expressed as
% \begin{equation}
%     \Grid_{\Rad,ijk} = \sum_{r=1}^{R} \Vector_{\Rad r,i}^{X} \Matrix_{\Rad r,jk}^{YZ} \AppVec_{r,p} + \Vector_{\Rad r,j}^{Y} \Matrix_{\Rad r,ik}^{XZ} \AppVec_{r,p} + \Vector_{\Rad r,k}^{Z} \Matrix_{\Rad r,ij}^{XY} \AppVec_{r,p}. 
%     \label{eqn:rad-vmr}
% \end{equation}
\begin{align}
    \Grid_{\Rad} = \sum_{r=1}^{R_\Rad}& \Vector_{\Rad, r}^{X} \OuterP \Matrix_{\Rad,r}^{YZ} \OuterP \AppVec_{3r-2} + \Vector_{\Rad,r}^{Y} \OuterP \Matrix_{\Rad,r}^{XZ} \OuterP \AppVec_{3r-1} \notag \\
    &+ \Vector_{\Rad,r}^{Z} \OuterP \Matrix_{\Rad,r}^{XY} \OuterP \AppVec_{3r}. 
    \label{eqn:rad-vmr}
\end{align}

Overall, we factorize the entire tensorial radiance field into $3R_\Dens+3R_\Rad$ matrices ($\Matrix_{\Dens,r}^{YZ}$,$...$,$\Matrix_{\Rad,r}^{YZ}$,...) and $3R_\Dens+6R_\Rad$ vectors ($\Vector_{\Dens, r}^{X}$,...,$\Vector_{\Rad, r}^{X}$,...,$\AppVec_r$). 
Each tensor element $\Grid_{\Dens,ijk}$, $\Grid_{\Dens,ijkp}$ are computed by
\begin{align}
    \Grid_{\Dens,ijk} =  \sum_{r=1}^{R_\Dens} & \Vector_{\Dens,r,i}^{X} \Matrix_{\Dens,r,jk}^{YZ} + \Vector_{\Dens,r,j}^{Y} \Matrix_{\Dens,r,ik}^{XZ} \notag \\
    & + \Vector_{\Dens,r,k}^{Z} \Matrix_{\Dens,r,ij}^{XY} \label{eqn:dens-vmrelement} \\
    \Grid_{\Rad,ijkp} =  \sum_{r=1}^{R_\Rad} & \Vector_{\Rad,r,i}^{X} \Matrix_{\Rad,r,jk}^{YZ} \AppVec_{3r-2,p} + \Vector_{\Rad,r,j}^{Y} \Matrix_{\Rad,r,ik}^{XZ} \AppVec_{3r-1,p} \notag\\
    & + \Vector_{\Rad r,k}^{Z} \Matrix_{\Rad r,ij}^{XY} \AppVec_{3r,p}. 
    \label{eqn:rad-vmrelement}
\end{align}
Here $i$,$j$,$k$ are indices for the XYZ modes and $p$ is the feature channel index.
In general, we adopt $R_\Dens \ll I, J, K$ and $R_\Rad \ll I, J, K$, leading to a highly compact representation that can encode a high-resolution dense grid.

\subsection{Efficient feature decoding.}
% Radiance field rendering is based on ray marching that requires sampling a lot of 3D locations and computing their density values and view-dependent colors.
% This desires our representation to efficiently compute the volume features at any 3D locations.
% Note that, with our factorized representation, any element value of the original tensors can already be evaluated at very low costs; as shown in Eqn.~\ref{eqn:vmrelement},  computing one tensor element only requires indexing one value per (vector or matrix) factor and combining them with simple multiplications and additions.
Note that, as shown in Eqn.~\ref{eqn:dens-vmrelement} and \ref{eqn:rad-vmrelement}, our model already allows for each tensor element to be evaluated at very low costs, requiring indexing only one value per (vector or matrix) factor and combining them with simple multiplications and additions.
% The original tensors represent discrete feature data. 
We further enable efficient trilinear interpolation for our model, enhancing the spatial coherence and leading to a continuous field. 
Moreover, since the shading function ($\ShadFunc$, discussed in Sec.~\ref{sec:grids}) always requires a full $\DimCh$-channel feature vector to compute view-dependent color, 
we also introduce a simple technique to efficiently obtain a full feature vector, without requiring computing individual channels separately as Eqn.~\ref{eqn:rad-vmrelement}.

To ease the following discussion, we also denote tensor components $\Comp^X_r=\Vector_r^X \OuterP \Matrix_r^{YZ}$, $\Comp^Y_r=\Vector_r^Y \OuterP \Matrix_r^{XZ}$, and $\Comp^Z_r=\Vector_r^Z \OuterP \Matrix_r^{XY}$; here the superscripts XYZ over $\Comp$ are for separating different components.


\paragraph{Trilinear interpolation.}
Naively achieving trilinear interpolation for our tensorial model requires first recovering 8 corner tensor elements (using Eqn.~\ref{eqn:dens-vmrelement} and \ref{eqn:rad-vmrelement}) and then interpolating them trilinearly. This increases 8x computation and memory costs compared to computing a single tensor element. 
However, we find that trilinearly interpolating a tensor data along its three modes is naturally equivalent to interpolating its vector/matrix factors linearly/bilinearly for the corresponding modes.

For example, given a component tensor $\Comp_r=\Vector_r^X \OuterP \Matrix_r^{YZ}$, we already know $\Comp_{r,ijk}=\Vector_{r,i}^X \OuterP \Matrix_{r,jk}^{YZ}$ by definition, and now we also have
\begin{equation}
    \Comp_r(\Pos) = \Vector_r^X(x)\Matrix_{r}^{YZ}(y,z),
\end{equation}
where $\Comp_r(\Pos)$ is $\Comp_r$'s trilinearly interpolated value at location $\Pos=(x,y,z)$ in the 3D space, $\Vector_r^X(x)$ is $\Vector_r^X$'s linear interpolated value at $x$ along X axis, and $\Matrix_{r}^{YZ}(y,z)$ is $\Matrix_{r}^{YZ}$'s bilinearly interpolated value at $(y,z)$ in the YZ plane. Therefore, we can efficiently compute trilinearly interpolation with a few linear and bilinear interpolation on the vector and matrix factors.

\paragraph{Feature vector.} We re-write a simplified 1D-slice version of Eqn.~\ref{eqn:rad-vmrelement}
\begin{align}
    \Grid_{\Rad,ijk} =  \sum_{r=1}^{R_\Rad} \Comp^X_{\Rad,r,ijk} \AppVec_{3r-2} + \Comp^Y_{\Rad,r,ijk} \AppVec_{3r-1}
     + \Comp^Z_{\Rad,r,ijk} \AppVec_{3r}. 
    \label{eqn:rad-vmrslice}
\end{align}
Here $\Grid_{\Rad,ijk}$ is a 1D slice along the feature dimension fixing the indices $ijk$, corresponding to the feature vector at $ijk$. 
This equation corresponds to the actual computation required by computing a single feature vector. 
We reduce the computational costs for computing a large number of feature vectors in parallel by simply re-ordering Eqn.~\ref{eqn:rad-vmrslice}.

We use $[\Comp_{\Rad,ijk}]$ to denote the vector that stacks all $\Comp^\star_{\Rad,r,ijk}$ values for $\star=X,Y,Z$ and $r=1,...,R_\Rad$, which is of $3R_\Rad$ dimensions.
We also stack all vectors $\AppVec_r$ as columns into a $P\times 3R_\Rad$ matrix $\AppMat$.
Then, computing equation~\ref{eqn:rad-vmrslice} is equivalent to computing
\begin{align}
    \Grid_{\Rad,ijk} =  [\Comp_{\Rad,ijk}] \AppMat^T. 
    \label{eqn:rad-vmrfeature}
\end{align}
Note that, since $\AppMat^T$ is completely separated from computing $\Comp^\star_{\Rad,r,ijk}$, we can now compute $[\Comp_{\Rad,ijk}]$ for all feature vectors and multiply $\AppMat^T$ once.



